Predicting Political Ideology from Digital Footprints

This paper proposes a new method to predict individual political ideology from digital footprints on one of the world's largest online discussion forum. We compiled a unique data set from the online discussion forum reddit that contains information on the political ideology of around 91,000 users as well as records of their comment frequency and the comments' text corpus in over 190,000 different subforums of interest. Applying a set of statistical learning approaches, we show that information about activity in non-political discussion forums alone, can very accurately predict a user's political ideology. Depending on the model, we are able to predict the economic dimension of ideology with an accuracy of up to 90.63% and the social dimension with and accuracy of up to 82.02%. In comparison, using the textual features from actual comments does not improve predictive accuracy. Our paper highlights the importance of revealed digital behaviour to complement stated preferences from digital communication when analysing human preferences and behaviour using online data.

==> Abstract.tex <==
% https://www.monash.edu/graduate-research/examination/publication
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis/writing-the-thesis-chapters/structuring-a-long-text
\abstract{
\addtocontents{toc}{}  % Add a gap in the Contents, for aesthetics

We utilize an original data set from Reddit that contains labels of self-described political ideology for 91,000 Reddit users along with records of the frequency with which they post in over 190,000 different sub-forums (subreddits) and the textual content of their comments to build predictive models that map digital footprints to political ideology.  We validate existing findings with our new data set and then leverage our sophisticated response variable, which indicates both the `social' and economic component of users’ political ideology, and allows for centrist self-identification on one or both dimensions, to  make several novel contributions to our understanding of how digital footprints can predict ideology. We find that the economic dimension of ideology can be predicted to a high degree  of accuracy and that this result is robust to the inclusion of those with self-identified centrist economic views. Contrastingly, our models are unable to accurately predict the `social' dimension of users’ ideologies. We also find that records of digital interactions are stronger predictors of ideology than online comments and discuss why this finding  may be idiosyncratic to our data. We briefly discuss the policy implications of our findings. 

\textbf{Keywords:} data mining, political ideology, digital footprint, online privacy, Reddit 
}


==> Acknowledgements.tex <==
% https://www.monash.edu/graduate-research/examination/publication
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis/writing-the-thesis-chapters/structuring-a-long-text
\ack{
\addtocontents{toc}{}  % Add a gap in the Contents, for aesthetics

Greatest thanks to Professor Paul Raschky for agreeing to supervise this unconventional and ambitious project and for providing valuable feedback and advice, as well as access to the SoDa Labs research group. On that note, many members of SoDa Labs deserve thanks for providing insightful commentary on initial findings which helped further develop this project. I would also like to thank Professor Heather Anderson for her feedback and advice as coordinator of the honours program. Thanks also to Sophie, Fraser and Stephen for providing careful proof readings of early drafts. 

This project was completed using a large number of Python and R packages which are listed and, where applicable, cited in Appendix \ref{Appendix-software}.


}

==> Chapter1.tex <==
\chapter{Introduction}
\label{Introduction}

Privacy concerns regarding online data have become increasingly prevalent in the wake of several high profile social media privacy scandals in recent years, most notably the Facebook-Cambridge Analytica data scandal\footnote{Cambridge Analytica boasts of dirty tricks to swing elections. \textit{The Guardian}, 2018, \url{https://www.theguardian.com/uk-news/2018/mar/19/cambridge-analytica-execs-boast-dirty-tricks-honey-traps-elections} (accessed 21 October 2021).}. Of particular concern is the threat that we can inadvertently reveal private traits through seemingly innocuous online behaviour. This has serious real world implications. Consider the possibility of someone’s sexuality being accurately determined from records of their online activity. In countries with conservative attitudes towards sexuality, people with non-traditional sexual orientations could be at risk of having their sexuality exposed and being subject to prejudice and harm. 

Consequently, there is a growing body of academic work devoted to predicting the traits of individuals (personality, gender, sexuality, etc.) on the basis of their digital footprints. Understanding the extent to which such prediction is possible informs the appropriate level of concern that should be paid to matters of digital privacy policy. Existing work has largely focused on psychological (e.g. Big Five personality traits) and demographic traits (e.g. gender). Pioneers in linking traits to digital behaviour relied on volunteers granting access to their social media information and were thus constrained to relatively small sample sizes\cite{Ross2009, Amichai-Hamburger2010, Golbeck2011a, Gosling2011}. More recently, researchers have begun using larger data sets with thousands of users or posts as the basis of analysis to make more robust findings. It has been shown that sexual orientation can be accurately predicted from pictures of an individual’s face using neural networks\cite{wang2018deep} and that Facebook Likes can accurately predict Big Five personality traits, gender, race, drug use and other traits\cite{kosinski2013private}. Even high level features of a Facebook profile (number of friends, number of statuses posted) have been shown to correlate with and predict personality\cite{10.1145/2380718.2380722}. 

Indeed, it has been found that digital footprints can be used to train statistical models capable of predicting people’s personality traits to a higher degree of accuracy than their close friends and family\cite{youyou2015computer}. Publicly available information from Twitter profiles\cite{Golbeck2011, Quercia2011} and Facebook messages\cite{Schwartz2013} has also been used to predict psychological traits using natural language processing techniques. Meta analyses claim that “the predictive power of digital footprints over personality traits is in line with the standard “correlational upper-limit” for behavior to predict personality”\cite{Azucar2018} and that “digital traces from social media can be studied to assess and predict theoretically distant psycho-social characteristics with remarkable accuracy”\cite{settanni2018predicting}. Further, it is not only digital traces from social media that can be effectively employed to predict private traits. The word choices of blog writers\cite{Yarkoni2010},  the images `favorited' by Flickr users\cite{Segalin2017} and mobile phone usage data\cite{stachl2020predicting} have also been fruitfully applied to this end. These sorts of models can be effectively used to persuade people. Facebook advertisement with messages tailored towards predicted personality types, as indicated by Facebook Likes, increases engagement with advertised content\cite{Matz2017}.
 
% BACK TO CHAP 1  

Political ideology has received relatively less focus. However, the accurate prediction of ideology from digital footprints could be misused to the detriment of society in several ways. If it is possible to accurately predict an individual’s ideology from their digital behaviour (even digital behaviour that is not of an explicitly political nature) then individuals with democratic sympathies living in authoritarian regimes may inadvertently reveal their non-conforming political views through ostensibly harmless online behaviour and be at risk of government retaliation. Additionally, the possibility of accurately estimating ideology may enable and encourage online political micro-targeting strategies aimed at voter suppression, which are considered to be in opposition with a functional liberal democracy by some\cite{anderson2018one}. 

This paper seeks to further illuminate the extent to which digital footprints can predict political ideology by leveraging an original data set to predict economic and `social' ideology, using textual and non-textual digital footprints, in a multi-class classification problem that allows for centrist self-identification. We have scraped the usernames and political ideologies of 91,000 users active on Reddit, one of the largest social news and discussion platforms globally. We have also recorded the frequency with which (most of) these users comment and post in a range of interest based discussion sub-forums (`subreddits') as well as the textual content of around 100 comments per user. With this data, we modelled the political ideology of these users as a function of the extent to which they engage with different subreddits and the textual content of their comments.  Section \ref{Data} of this paper provides further information on our data. Section \ref{Methodology} details the modelling strategies we employ. 

Ideology has been paid some attention in the literature on predicting  private traits from digital footprints. It has been illustrated that natural language processing techniques can be used to accurately classify the political leanings of Twitter users\cite{colleoni2014echo, Conover2011, Makazhanov2013, Boutet2012} and their political engagement or ideological extremity\cite{Preotiuc-Pietro2017}. Hashtags and network analyses of mention/retweet networks can also be leveraged to effectively classify the ideologies of Twitter users\cite{Conover2011, Barbera2015, Boutet2012}. Kosinski et al.'s seminal work\cite{kosinski2013private} pays some attention to political traits. Kosinski et al. map the Likes of 9,572 American Facebook users with a self-disclosed party affiliation of  either Democrat or Republican using a logistic regression model, illustrating that the model’s predictions on unseen data achieve an ROC-AUC (receiver operating characteristic, area under curve) of 0.85. Our approach to modelling ideology as a function of digital footprints is broadly based on the methods used in this paper. 

This body of work represents a great leap in our understanding of how online behaviour can be leveraged to predict ideology. However, some important questions remain unanswered. Firstly, the vast majority of these studies focus on predicting a binary variable representing ideology (for a systematic literature review see \cite{Hinds2018}). In reality, ideology is not binary and many people identify as centrists so we want to know if the accurate prediction of ideology is robust to the inclusion of centrists. Some research has been done into multi-class prediction of ideology but these studies rely on textual\cite{Boutet2012, Makazhanov2013, Preotiuc-Pietro2017} and network data\cite{Boutet2012, Barbera2015}  which does not generalise to ubiquitous footprints like web search logs, and sometimes utilise fallible ground truths\cite{Makazhanov2013, Preotiuc-Pietro2017}. Secondly, a one-dimensional conception of ideology is typically insufficient to capture people's political beliefs. Many people consider themselves socially progressive but fiscally conservative and cannot easily be placed into a simple left/right spectrum. Consequently, we want to know whether some dimensions of ideology are more readily predictable than others. We have not identified any studies that attempt to answer this question. Finally, it is unclear if textual or non-textual digital footprints (Facebook Likes, search history logs, etc.) are better predictors of ideology. Again, to our knowledge no study has directly compared the predictive power of textual and non-textual footprints that mimic a broader range of footprints.

We utilise a sophisticated measure of ideology in our original data set, which allows for centrist self-identification (on both the economic and `social'\footnote{The term `social' for this ideological dimension is somewhat misleading, we provide a fuller explanation of what is meant here in Section \ref{Data}.} dimensions of ideology), to contribute to the literature by answering the three open questions outlined above. Firstly, we test if the accurate prediction of ideology from digital footprints is robust to the inclusion of self-identified centrists. In a similar vein, we also illustrate how the quality of predictions is affected by the complexity of the ideological variable we seek to model. Further, we decompose users' ideologies into both an economic component and `social' component, allowing us to investigate whether the economic component of political ideology is more readily predictable than the `social' component. Finally, we model ideology using as features the frequency of users' interactions with subreddits, the textual content of their texts and the union of these sets of features. This provides insight into what sorts of digital footprints are most informative with respect to ideology. Our findings have important policy upshots that we discuss in Section \ref{Discussion}. 

Our research also illustrates the usefulness of Reddit data in the study of political ideology. Data from Reddit has been used to predict personality and gender\cite{Gjurkovic2020}, and even detect mental illnesses like anxiety, depression and schizophrenia\cite{Kim2020}. However,  a systematic review of the literature on linking digital footprints to political orientation indicates that no one has previously used Reddit data to this end\cite{Hinds2018}. By showing Reddit to be a reliable source of rich social data we hope to spur further developments in this field.

We find that economic ideology is readily predictable from digital footprints and that this result is robust to the inclusion of self-identified economic centrists, although model performance diminishes significantly when centrists are included. Contrastingly, our models are unable to predict `social’ ideology at levels significantly above performance baselines. We also show that classification of a complex dependent variable representing nine different ideological classes can be achieved with a level of accuracy above baseline levels. In all cases, the frequency of interactions with different subreddits (analogous to digital footprints like search logs, purchase histories, etc.) is a stronger predictor than the textual content of comments and the union of both sets of features only marginally improves performance. We provide a fuller account of our results in Section \ref{Results}. 

We note that modelling ideology as a function of digital footprints is, in part, provided for by the fact that an individual’s latent psychological makeup drives both their online behaviour and their political beliefs. Importantly, this provides for the observed association between online behaviour that is not of an explicitly political nature and ideological views (posting in Marxist or conservative discussion forums would constitute explicitly political online behaviour). This is central to the privacy concerns we wish to illuminate. It is the fact that digital behaviour of an entirely non-political nature can imply ideology that is cause for concern; for instance, as we show later,  frequently using the word `feel' in online comments is strongly associated with economically left wing views. As such, we provide a brief overview of the psychological foundations of ideology and of digital behaviour.

There is a demonstrated association between psychological traits and certain interests\cite{Wolfradt2001, McCrae1997}. Interests likely impact language use (if you like movies you probably use words like `actor' and `film' a lot) and people with certain interests are more likely to participate in online forums pertaining to these interests. 

Psychological traits also influence ideology. There is a substantive amount of literature in psychology that has focused on modeling ideology as a function of scores on particular psychometric scales. In one study, the Big Five model of personality was used to predict party preferences in Italy, Spain, Germany, Greece and Poland\cite{Vecchione2011}. It was found that Big Five traits were more powerful predictors than demographic characteristics (age, gender, income, education) and that openness to experience predicts left wing views whilst conscientiousness predicts voting for conservative parties. They note that the linkage between personality and political views is consistent with theoretical expectations: conscientiousness comprises a preference for order and adherence with rules whereas openness to new ideas correlates against preferences for rigid social hierarchy\cite{Vecchione2011}. It has been shown that including scores from the HEXACO model of personality as additional regressors alongside Big Five traits increases the proportion of variance explained when modeling ideology\cite{Chirumbolo2010}. Another study illustrates that scores on Hartmann’s Boundaries Questionnaire can predict conservatism\cite{Hiel2004}. Some results are consistent with theoretical expectations; conservatism is correlated with a preference for rigid and well defined social structures, whilst other results are harder to explain; conservatism is also positively correlated with a preference for blurred edges and soft lines in art. 

More broadly, a meta analysis of ``conservatism as a function of social cognition" has found that death anxiety, system instability, dogmatism, openness to experience, uncertainty tolerance, need for order, structure and closure, integrative complexity, fear of threat and loss and self-esteem all have predictive power of conservatism\cite{Jost2003}. Consider how an individual’s interests and activities are likely influenced by these traits. Someone with substantial death anxiety may resultingly have a strong interest in existential philosophy. Someone with low openness to experience may prefer older, familiar television shows to more recent ones. Consequently, psychological traits influence both ideology and our interests, which in turn influences our online behaviour, providing for an observable mapping of online behaviour to ideology which can be approximated by statistical learning models. 














%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%










==> Chapter3.tex <==
\chapter{Data}
\label{Data}



To fill the gaps in the literature discussed in Section \ref{Introduction}, we require digital footprints and multi-dimensional ideological labels from a large number of internet users. Finding such data is not a trivial task. The MyPersonality data set that contains information on a large number of Facebook users' Facebook Likes is no longer available (nor does it contain sufficiently sophisticated ideological labels) and obtaining new data from Facebook is not realistic due to Facebook's increased protection of private data in response to privacy scandals. Twitter, whilst a viable source of data for such inquiry, is limited by the fact that there is no real way to effectively and easily collect information on the ideologies of large amounts of users. Further, using purely textual data (like Tweet data) will only allow us to predict ideology as a function of explicit textual communication. We would, however, also like to get an indication of how more subtle digital footprints that do not involve explicit communication can be used to predict ideology.

We opted to scrape an original data set from the  \href{https://www.reddit.com/r/PoliticalCompassMemes/}{r/PoliticalCompassMemes} subreddit, a Reddit forum in which users `humorously' critique ideologies in opposition to their own. In this subreddit, users ‘flair’ their posts with with their results from the popular \href{https://www.politicalcompass.org/test}{Political Compass Test}. We created a Python script using the Python Reddit API Wrapper (PRAW) library to scrape the r/PoliticalCompassMemes subreddit and collect the usernames, ideologies and post/comment histories of 91,000 users who had commented on posts in the subreddit. We also created a script using the PMAW Pushshift\cite{Baumgartner2020} API wrapper to collect a maximum of 100 comments from each user\footnote{This data is available upon request.}. \fref{fig.pcm-comment-fig} shows an example of how users' comments are flaired with their political ideology. \fref{fig.pcm-post-fig} shows a post from the subreddit in which a user flaired as conservative makes fun of U.S. President Joe Biden. \fref{fig.policompass-fig} shows the political compass; users are assigned to one of the four quadrants in the two-dimensional ideological space. 

\begin{figure}[!htbp]
\centering
  \fbox{\includegraphics[width=10cm,height=4.7cm]{Figures/pcm-comment-fig.png}}%
  \caption{A comment from a user who has flaired themselves as having economically right wing views and a response from a user who has flaired themselves as having a `libertarian left' ideology \label{fig.pcm-comment-fig}}
\end{figure}

\begin{figure}[!htbp]
\centering
  \fbox{\includegraphics[width=10cm,height=9.7cm]{Figures/pcm-post-fig.png}}%
  \caption{A post from a user who has flaired themselves as a member of the `authoritarian right' \label{fig.pcm-post-fig}}
\end{figure}


\begin{figure}[!htbp]
\centering
  \fbox{\includegraphics[width=10cm,height=9.7cm]{Figures/policompass-fig.png}}%
  \caption{The political compass. Flaired users take a test specifying the extent to which they agree with politically charged statements (e.g. ``If economic globalisation is inevitable, it should primarily serve humanity rather than the interests of trans-national corporations") and are assigned to one of four quadrants: libertarian left (social democrat), libertarian right (libertarian), authoritarian left (communist) or authoritarian right (traditional conservative) depending on their answers \label{fig.policompass-fig}}
\end{figure}

There were three steps to collating the data:

\begin{enumerate}
    \item Creating a list of usernames and ideology signaling flairs associated with each username.
    \item For each user in (1), going through their post and comment history and recording a tally of the amount of times they have posted and commented in each subreddit they interact with. 
    \item For each user in (1), collecting the textual content of the 100 most recent comments they have made in subreddits excluding r/PoliticalCompassMemes.
\end{enumerate}

The scripts used to perform all data scraping can be found in the \href{https://github.com/MichaelKitchener98/RedditIdeology-Honours2021/tree/main/data_collection}{data collection folder of the GitHub repository for this project}\footnote{\url{https://github.com/MichaelKitchener98/RedditIdeology-Honours2021/tree/main/data_collection}}.

Kosinski et al. note that findings from studies using Facebook Likes likely generalise to other types of digital footprints\cite{kosinski2013private}. The same is true of Reddit interactions. Reddit users are able to interact with millions of subreddits, which are interest or topic based discussion forums. As such, interaction with a subreddit can be seen as an expression of interest in the relevant topic (if a user interacts with the r/gaming subreddit, they are `showing' an interest in video games). Consequently, the frequency with which someone interacts with different subreddits is broadly analogous to other (likely richer) digital footprints such as web search logs (searching a topic also indicates interest in it)  so our results should generalise to the kinds of digital footprints that entities which threaten digital privacy have access to. 

\section{Creating a list of usernames and ideology signaling flairs}
\label{Data-creating-user-flair}

We created a list of usernames and associated ideology signaling flairs by running a Python script that cycled through the top 1,000 most popular posts of all time in the r/PoliticalCompassMemes subreddit. For each post, we looped through all the available comments. If the author of the comment was not already in a list of users whose ideology we had recorded and their comment was flaired with an ideology, we added their username and their flair as a row to the data set. The username was also added to the list of users whose ideology we had recorded to avoid doubling up. This resulted in a data set of 91,000 username and flair combinations. An illustration of this data can be found in \tref{table.user-flair-example}.

\begin{table}[!htbp]
\centering
\caption{Example user-flair data \label{table.user-flair-example}}
    \begin{tabular}{||c c ||} 
    \hline
    \textbf{username} & \textbf{ideology} \\ 
    \hline
    user1 &  Libertarian-Left \\
    \hline 
    user2 & Authoritarian-Right \\
    \hline
    user3 &  Libertarian-Right \\
    \hline
    \ldots & \ldots \\
    \hline
    \end{tabular}
\end{table}

There are a total of nine classes (different flairs that correspond to the same ideology were grouped together as detailed in Appendix \ref{Appendix-Recoding}). The \textbf{libleft} flair corresponds to social democrats, i.e. supporters of Bernie Sanders,  \textbf{libright} to libertarians, i.e. supporters of Ron Paul, \textbf{libcenter} to those who identify as libertarians with respect to the role of the state in social matters but have centrist economic views, \textbf{centrist} to  those who identify as having centrist views on the economy and the role of the state in social matters, \textbf{left} to those who identify as having left wing economic views but centrist views on the role of the state in social matters, \textbf{right} to those who identify as having right wing economic views but centrist views on the role of the state in social matters, \textbf{authright} to  traditional conservatives, i.e. supporters of Ted Cruz, \textbf{authleft} to communists, i.e. supporters of Xi Jinping and \textbf{authcenter} to those who identify as having authoritarian views with respect to the role of the state in social matters but centrist (or perhaps mixed) economic views\footnote{This ideology is treated as a pro-fascism ideology in the forum.}. The frequency and sample proportion of each ideological class is described in \tref{table.response-freq-prop} and illustrated in \fref{fig.response-freq}.

%{|r|r|r|r|r|r|r|r|r|r|}
\begin{table}[!htbp]
\centering
\caption{Ideology frequency and proportion in sample (n = 91,000) \label{table.response-freq-prop}}
\scalebox{0.8}{\begin{tabular}[t]{||r r r r r r r r r r||}
\hline
 & libleft & libright & libcenter & centrist & left & right & authright & authcenter & authleft\\
\hline
Frequency & 18,070 & 15,054 & 13,548 & 13,408 & 9,646 & 6,526 & 5,672 & 4,801 & 4,275\\
\hline
Proportion & 0.2 & 0.17 & 0.15 & 0.15 & 0.11 & 0.07 & 0.06 & 0.05 & 0.05\\
\hline
\end{tabular}}
\end{table}

\begin{figure}[!htbp]
\centering
  \fbox{\includegraphics[width=14cm,height=8.75cm]{Figures/response_freq.pdf}}%
  \caption{Ideology frequency in sample ($n = 91,000$), note: we were unable to gather footprints for some users so the size of the data set that is used in model training varies depending on the particular model \label{fig.response-freq}}
\end{figure}

The Political Compass Test only allocates users to one of four quadrants (authleft, authright, libleft, libright) by providing quantitative scores of how right or left they are economically and how libertarian or authoritarian they are `socially'. Presumably, users who identify as, say, `left' have taken the test and found that though they score highly `left' in the economic dimension, they are only marginally above or below the origin (midpoint) of the `social' axis. Likewise, centrist users may consider themselves insufficiently far from the origin in either dimension to warrant any other classification. Still, it is fundamentally up to the discretion of the user as to whether to identify in accordance with their test outcome or as a  centrist on one or both ideological dimensions. This choice may be based on prior beliefs regarding their political views. Consequently, the labels here must fundamentally be understood as self-reported ideologies rather than as results from the test even though these self-reported ideologies are presumably strongly influenced and calibrated by test results.

In what follows we refer to users' position on the left/right axis as economic ideology (position here is defined by responses to questions regarding the economy) and position on the authoritarian/libertarian axis as social ideology. It may not be immediately clear how the terms authoritarian/libertarian relate to `social' political ideology but inspection of the relevant questions on the Political Compass Test reveals that these questions elicit preferences for government's coercive involvement in social facets of life, i.e. whether the government should enforce a ban on abortion. As such the term `social' ideology provides a useful shorthand that will be employed in the remainder of this paper (with the omission of single quotation marks). 

There is no guarantee that each username in our data set corresponds to a unique person; one individual could have two or more different Reddit accounts. However, this is unlikely to be a prevalent behaviour and should have a negligible effect on the validity of our data. It is also possible that an account’s flair may not truly represent the ideology of the person behind the account. This could be due to users mistakenly assuming that they subscribe to a particular ideology without having taken the test to calibrate their self-assessment. It is also possible that some users create accounts flaired with ideologies other than their own in order to post stereotypes associated with adherents of that ideology in an effort to satirise the beliefs of their ideological opponents. We do not consider this a substantive issue in our data.

\section{Collecting the subreddit interaction records of flaired users}
\label{Data-collect-digital-footprint}

With the user-flair data collected, the next step was to obtain comprehensive digital footprints for all of the users whose ideology was known. For each user, we looped through their 1,000 most recent posts and 1,000 most recent comments. Each post or comment was stored as a row in a data set with the following columns: \textbf{user:} the username of the user whose posts/comments we are recording; \textbf{interaction:} whether the interaction being recorded is a comment or a post; \textbf{title:} the title of the post if the interaction is a post, otherwise blank; \textbf{score:} the `score' of the post/comment; other users can `upvote' a post or comment and increase its score by 1 or `downvote' the post or comment and decrease its score by 1; \textbf{time:} the time the post/comment was created; \textbf{subreddit:} the subreddit the post/comment was made in.


A hypothetical illustration of this data can be found in \tref{table.user-history-example}.

\begin{table}[!htbp]
\centering
\caption{Example user-history data \label{table.user-history-example}}
\scalebox{1}{\begin{tabular}{||c c c c c c||} 
\hline
\textbf{username} & \textbf{interaction} & \textbf{title} &  \textbf{score} & \textbf{time} & \textbf{subreddit} \\ 
\hline
user1 &  post & GTA V \dots &  43 & 10:32 2/1/21 & r/gaming  \\
\hline 
user1 &  comment &  & 12 & 16:12 8/12/20 & r/classicalmusic \\
\hline 
user2 &  post & Today's \dots &  -6 & 5:36 4/3/21 & r/boxing \\
\hline 
user2 &  post & The \dots &  3 & 4:24 4/3/21 & r/seinfeld \\
\hline 
user2 &  comment &  &  0 & 5:09 3/3/21 & r/crypto \\
\hline 
\ldots & \ldots & \ldots      & \ldots  & \ldots  & \ldots \\
\hline
\end{tabular}}
\end{table}

This can be transformed into a user-interaction matrix where each row represents a unique user and each column refers to a particular subreddit. The value in any particular cell can represent a number of things: the number of times the user has posted/commented in that subreddit, whether the user has posted/commented in that subreddit or the average score of the user’s posts/comments in that subreddit. \tref{table.user-interaction-example} illustrates what a user-interaction matrix may look like.

\begin{table}[!htbp]
\centering
\caption{Example user-interaction matrix \label{table.user-interaction-example}}
\begin{tabular}{||c c c c c||} 
\hline
\textbf{username} & \textbf{r/gaming} & \textbf{r/classicalmusic} & \textbf{r/boxing} & \textbf{r/seinfeld} \\ 
\hline
user1 &  3 & 12 & 0 & 0 \\
\hline 
user2 &  0 & 4 & 1 & 6 \\
\hline 
user3 &  0 & 0 & 0 & 0 \\
\hline 
user4 &  1 & 0 & 0 & 14 \\
\hline 
user5 &  0 & 43 & 0 & 0 \\
\hline 
\ldots & \ldots & \ldots   & \ldots   & \ldots  \\
\hline
\end{tabular}
\end{table}

The user-interaction matrix is a set of predictors for each user and can be merged with the user-flair data. This allows us to model ideology as a function of digital interactions. As described in Section \ref{Methodology-user-interaction}, to examine the extent to which ideology may inadvertently be revealed, we removed columns that represent interactions with explicitly political subreddits when developing predictive models. Since there are a huge number of (debatably) political subreddits we are unable to remove all of them, however, by removing the many of the most popular political subreddits we hope to minimise the influence of explicitly political subreddits on our models. Appendix \ref{Appendix-removed} lists the subreddits which we removed from the user-interaction matrix when modelling. 

The user-history data set is very large (63,709,041 rows) so transforming it into a user-interaction matrix is not a trivial computational task. The user-history data is pivoted chunk by chunk. The final user-interaction matrix comprises the union of all chunks. We transformed the user-history data set into a user-interaction matrix where each cell represents the amount of times the user has posted or commented in the relevant subreddit. 

It should be noted that the limit of 1,000 posts/comments is not arbitrary. PRAW limits requests to 1,000 objects at a given time; i.e. if we are looping through a particular subreddit’s top posts we can at most request 1,000 post objects from PRAW. It was on this basis that we elected to gather usernames and flairs through the top posts since these are likely to have many comments and hence more user/flair combinations to record. We also chose to record each user's 1,000 most recent posts and comments as these are presumably most reflective of the user's most current attitudes and interests. There may not be exactly 1,000 records returned from any request since deleted posts may be returned and contribute to the request limit despite being of no use to us. We discuss associated issues for our study in Section \ref{Data-caveats}.

If our user-history script encountered an error whilst collecting records of subreddit interactions for a given user (this could happen occasionally, often due to issues with Reddit's servers) it disregarded all data collected for that user and skipped to the next user to avoid censoring records of interactions for specific users.

\section{Collecting the comments of flaired users}
\label{Data-collect-comments}

We looped through each user in our list and recorded their 100 most recent comments from any subreddit excluding r/PoliticalCompassMemes. The process of extracting features to use in our models from this raw textual data is described in Section \ref{Methodology-text}.

In the user-interaction matrix, we removed interactions with popular, explicitly political subreddits from our set of features. We do not remove explicitly political words (i.e. words that may be associated with partisanship) as there is no way to a priori determine how the use of politically charged words discloses ideology. For instance, a progressive may use the words ‘Trump’ and ‘gun’ a lot as they criticise the Trump administration and lack of stringent gun control in the United States. That is to say, the use of these politically charged words does not explicitly disclose an ideological viewpoint (as we assume participation in explicitly ideological subreddits to). Consequently, we do not remove any words from our corpus. 

We could have avoided scraping comments from our list of politically explicit subreddits but there is no reason to think that the language used in these subreddits constitutes an explicit disclosure of ideology. Knowing the textual content of a comment in an explicitly political subreddit without knowing what the subreddit actually is, is insufficient information to infer ideology. Consider the following analogy, if someone tells you that they spend last Thursday night at their local Labor Party branch meeting then they are effectively disclosing their political beliefs to you. If they tell you they spend last Thursday night talking about Federal Parliament and trade unions (whilst at a Labor Party branch meeting, though they do not tell you this) they have not definitively revealed their political beliefs.

The scraper occasionally encountered errors whilst collecting comment data. When this happened, we used an error catch to drop all data for the user whose data we were collecting when the error occurred (to avoid censoring the textual content of comments for specific users) and skipped to scraping the comments of the next user in our list.

\section{Caveats}
\label{Data-caveats}

There are some caveats common to all research with digital data that should be mentioned. As noted, our subreddit interaction records for a given user are limited by Reddit’s API. We also only recorded the textual content of a maximum of 100 comments per user due to computational restrictions. Such issues are endemic to data scraped from the web where API limits often restrict how much data can feasibly be extracted for each user. 

Further, our sample is not representative of any particular national population. Users may come from any country (although most appear to come from English speaking countries). The distribution of key demographic variables like age, education, income and race in the population of Reddit users is likely far less varied than it is in any country level population. Further, users who comment and flair themselves in the r/PoliticalCompassMemes subreddit likely have different traits to the broader population of Reddit users. Clearly, there are major sample selection issues here. We are not attempting causal inference but there is a risk that the average r/PoliticalCompassMemes commentor has a greater interest in politics than the average Reddit user. This may manifest in greater engagement with activities (and hence subreddits) which are strongly associated with particular ideologies as ideology is a larger part of personal identity for these people. As such, our model may over estimate the predictive accuracy of digital footprints over political views and our findings/models may not generalise to predicting the ideologies of less politically engaged users whose interests (and digital interactions) are less tied to their political views. However, these selection effects may also deflate the observed associations between predictors and response, causing our models to understate the predictive power of digital footprints. The sample selection effects constrain the range of the distributions of our predictors (people who interact with the r/PoliticalCompassMemes subreddit likely have a narrower range of interests and hence subreddit use and language variation than the broader Reddit population) and accordingly reduce the variance in our predictors that can correlate with our response variable. We note that this sample selection issue is common in all studies focused on predicting private traits through digital records, many of which feature selection bias by requiring users to voluntarily disclose relevant traits\cite{kosinski2013private, 10.1145/2380718.2380722, colleoni2014echo, youyou2015computer, Golbeck2011, Quercia2011, Preotiuc-Pietro2017}.

Another potential issue comes from how we collected users' ideologies as signalled by their flairs at time $t_1$ but scraped their most recent comments at time $t_2$ where $t_2 > t_1$. If a user's ideology has changed between $t_1$ and $t_2$ then their digital footprints may not reflect the digital behaviour associated with their flaired ideology, undermining predictive models. We do not consider this to be a substantive risk  
as the subreddit has only been popular for a few years so there is typically a relatively short interval between the creation of flaired comments and the collection of digital footprints.

\section{Advantages}
\label{Data-advantages}

The previous section elaborates on the limitations of our data that are, by and large, endemic to all research in this field. However, our data also promises several advantages over that used in previous studies. We will describe the advantages of our data with reference to the MyPersonality data set used by Kosinski et al.\cite{kosinski2013private} since this work provides the methodological basis of our paper. The MyPersonality data set features records of the Facebook Pages ‘Liked’ by over 58,000 Facebook Users who agreed to take an online personality survey and have data collected from their Facebook profile. The data set also contains the US party affiliation of 9,572 Facebook Users who declared this information on their profile. 

As noted, we want our data to proxy a broader range of digital footprints so that we can understand just how salient digital privacy concerns are. Facebook Likes and Reddit interactions data are both reasonable proxies of  web search logs, purchase records, and other digital footprints. However, we propose that Reddit data better emulates these footprints for several reasons.

Firstly, due to the anonymity of Reddit relative to Facebook, users may be more willing to implicitly disclose private interests via digital behaviour (users may comment in certain pornographic subreddits but few people would willingly disclose this information via their Facebook Likes). These private interests may correlate with ideology. The fact that Reddit data captures this kind of information makes it a better proxy: consider how people typically use search engines under the presumption that their search queries are private. Essentially, Reddit data expresses the same range of interests as other digital footprints whereas Facebook data only expresses a restricted range of interests. 

Further, the MyPersonality data set relied on users reporting their political views on their Facebook profile (linked to their real life identity). As such, this data may suffer from a social desirability bias; people with political views that could be viewed unfavourably by their peers might decline to reveal them. The anonymity of Reddit means that r/PoliticalCompassMemes users do not have to worry about their ideologies being linked to their true identity and can freely reveal their political beliefs.

Our data also features a more sophisticated response variable than utilized by Kosinski et al. Our measure of ideology has two components corresponding to a two-dimensional conception of ideology. It also allows for users to identify as centrists on one or both dimensions. This enables us to make novel insights regarding the robustness of predictive accuracy when we include ideological centrists and the conduciveness of digital footprints to the estimation of different facets of ideology. 

Finally, our data set has 91,000 observations\footnote{In practice, some observations are removed from the training/testing sets for various reasons. The full amount of observations used in training, validating and testing each model is reported alongside metrics of model performance in Section \ref{Results-model}.} and is thus substantially larger than Kosinski et al.'s which features 9,752 observations with political labels.

==> Chapter4.tex <==
\chapter{Methodology}
\label{Methodology}

Firstly, we mapped the original flairs to {left, center, right} and removed centrists to perform binary classification on users' economic ideology. We also mapped flairs to {authoritarian, center, libertarian}, and removed centrists to perform binary classification on users' social ideology.  We refer to these classification problems as the economic problem and social problem respectively. Exact details on how we mapped from the set of nine classes to economic classes and social classes can be seen in Appendix \ref{Appendix-Recoding}.

The removal of centrist users can be justified on the basis that they may represent measurement noise. For instance, when we plot the data in singular value decomposition (SVD) component space, we typically see separations between right and left and (to a lesser extent) authoritarian and libertarian users. However, centrist users are randomly splattered throughout the SVD component space indicating that centrist users are not `true' centrists and may effectively be declining to reveal their true ideology. We illustrate this in \fref{fig.svd_scatter} and provide further demonstration in Appendix \ref{Appendix-svd}. 

Further, the existence of `true' centrists is debated in the political science literature; consider Duverger's proclamation: ``in politics, the centre does not exist"\cite{Brogan1955}. More concretely, recent work has tested competing hypotheses that attempt to explain why centrist self-identification arises. There is evidence that ``placing oneself on the center does not indicate that the individual is ‘ideologically centrist’"\cite{Rodon2015} but rather that centrist self-identification predominantly arises from individuals having insufficient political knowledge to place themselves on a left right scale (the \textit{uninterested hypothesis}) or individual's self-identification reflecting decisions to vote for centrist parties or candidates rather than genuine ideological centrism (the \textit{party-component hypothesis}). The \textit{uninterested hypothesis} clearly does not apply to users in our sample who willingly identify themselves as centrists and have an interest in politics but the \textit{party-component hypothesis} (and the empirical evidence supporting it) provides a compelling case to disregard those who have labeled themselves as centrists in our initial models. 

Finally, removing centrists allows for easier comparisons with the work of Kosinski et al.\cite{kosinski2013private} in which the US party affiliation of Facebook users (Democrat or Republican) is predicted, excluding all users that were not labelled as either. 

\begin{figure}[!htbp]
\centering
  \fbox{\includegraphics[width=14cm,height=8.75cm]{Figures/svd_scatterplot.pdf}}%
  \caption{Leftwing (magenta), rightwing (cyan) and centrist (grey) users from  the training and validation sets in SVD component space \label{fig.svd_scatter}}
\end{figure}

It is not for us to determine the legitimacy of centrist self-identification, so whilst we present the results of binary classification, and note that they may be meaningful in their own right, we also estimated these models again (for both the economic and social problem), this time including centrists. Results from this multi-class classification problem demonstrate whether the results of the binary classifications are robust to the inclusion of so-called `centrists’. We then estimated models for the full nine-class classification problem in which we attempted to classify users to a class from the full set of categories that feature in our ideological labels. 

For each classification problem we ran models where we used as features A) the user-interaction matrix, B) features extracted from the textual content of comments and C) the union of these sets of features. 

Our data was split into training (64\% of total data), validation (16\%) and testing (20\%) sets. In all models, hyperparameters were chosen according to accuracy on the validation set. We then retrained the model on the training and validation data using the optimal hyperparameters. We report the accuracy and, where applicable, the (weighted) ROC-AUC of all models' predictions on our testing set and present these results as indicators of the models' predictive power over ideology. Model accuracy and ROC-AUC are detailed in Section \ref{Methodology-model-assessment}.

We expect accuracy to decrease as the number of classes in the response variable increases. As such, we assess the accuracy of all models relative to the baseline accuracy of a ZeroR classifier, which assigns all observations to the plurality class in the training set. For example, in the nine-class classification problem, the ZeroR classifier assigns all observations to ‘libleft’ ($\sim$ 20\% of all observations in sample). If digital footprints can predict ideology then our models will exhibit accuracy greater than the accuracy of the ZeroR classifier on the testing set. The more accurate our models are over the ZeroR baseline, the stronger the evidence that digital footprints can predict ideology.

The code for the Scikit-Learn implementation of all models for which results are reported in Section \ref{Results} can be found in the  \href{https://github.com/MichaelKitchener98/RedditIdeology-Honours2021/tree/main/Models}{models folder of the GitHub repository for this paper}\footnote{\url{https://github.com/MichaelKitchener98/RedditIdeology-Honours2021/tree/main/Models}}.

\section{Methodology: user-interaction matrix}
\label{Methodology-user-interaction}

When using the user-interaction matrix as our set of features we removed popular, explicitly political subreddits from the user-interaction matrix prior to running the models. We also trimmed our user-interaction matrix to ensure that every user in the data set had made at least 50 comments and every subreddit had been commented in at least 50 times as suggested by Kosinski et al.\cite{Kosinski2016MiningBD}. This ensures that our user-interaction data better proxies digital footprints like search logs which are presumably expansive records. In many cases we `binarised' our data, i.e. for each cell $(i,\,j)$ of the user-interaction matrix, if $(i,\,j)$ is greater than 0 it was mapped to 1 in the binarised user-interaction matrix and 0 otherwise. The choice to binarise was made on the basis of validation set performance;  binarisation drastically increased performance for most models. 

In developing these models we followed the same broad approach as Kosinski et al.\cite{kosinski2013private}:

\begin{enumerate}
    \item Reduce the dimensions of our predictors via a SVD of our data matrix. A smaller feature set is generally conducive to better performing models.
    \item Train a supervised learning algorithm on the SVD components of the user-interaction matrix to classify the ideology of a user.
\end{enumerate}

In step 2 we used the following learning models for multi-class classification: one-versus-rest (OVR) logistic regression (with and without an $\ell_1$ penalty), multinomial logistic regression (with and without an $\ell_1$ penalty), random forests, OVR random forests and AdaBoost. In the binary case we exclude OVR schemes from all models and multinomial logistic regression reduces to standard logistic regression. A brief account of each model and the SVD is given in Section \ref{Methodology-overview-stat-learning} excluding (OVR) random forests and AdaBoosting as these supervised learning algorithms do not feature in our best model for any modelling problem. An overview of (OVR) random forests and AdaBoosting can be found in Appendix \ref{Appendix-methodology}. We used the Scikit-Learn Python package\cite{scikit-learn} to implement these models. 

\section{Methodology: text}
\label{Methodology-text}

We utilised two approaches to extracting features from the textual content of users' comments. Firstly, we created features corresponding to the term frequency-inverse document frequency of different terms in the concatenation of users' comments (tf-idf), where documents are the sets of different users' comments. Secondly, we used a Word2Vec model\cite{Mikolov2013, Mikolov2013a} that has been pre-trained on a Google News data set (`word2vec-google-news-300'\footnote{\url{https://drive.google.com/file/d/0B7XkCwpI5KDYNlNUTTlSS21pQmM/edit?resourcekey=0-wjGZdNAUop6WykTtMip30g}}) to convert the set of comments for each user into the simple average of the vector representations of their constituent words. 

We then  classified users' ideologies using a linear support vector classifier (SVC), applying a OVR scheme for multi-class problems. We restricted our choice of supervised learning algorithm to the linear SVC given that the strong performance of support vector machines in document classification is well established\cite{Joachims1998} (we did not experiment with non-linear kernel functions owing to computational constraints). 

We ran the SVC using A) tf-idf features, B) average Word2Vec features and C) the union of these two sets of features. Some models used a subset of SVD components from a SVD of the original features instead of the original features themselves (this decision was made on the basis of validation set performance). We outline tf-idf, Word2Vec as well as the linear SVC model in Section \ref{Methodology-overview-stat-learning}.

\section{Methodology: combined}
\label{Methodology-combined}

These models use both the (often binarised) user-interaction matrix and the tf-idf vectors as features. We scaled each feature to have the same range since tf-idf terms and user-interaction records are not on the same scale.
We then took a SVD of the data if validation set accuracy suggested that this increased performance. We then fed this data into an OVR logistic regression model  with an $\ell_1$ penalty and an OVR linear SVC (or just a simple logistic regression and linear SVC when dealing with binary classification problems). 

We did not use the full range of models experimented with earlier
because OVR logistic regression with an $\ell_1$ penalty typically performed very well for models taking the user-interaction matrix as features. Further, the union of tf-idf and average Word2Vec features leads to (at best) marginally better results than models that just use tf-idf features. 

\section{Model assessment}
\label{Methodology-model-assessment}

\subsection{Accuracy}
\label{Methodology-model-assessment-accuracy}

The accuracy of a model on a test set indexed by $i=1,\dots,n$ is given by:

$$\text{accuracy} = \cfrac{1}{n} \sum^n_{i=1} I(y_i = \hat{y}_i) $$ 

Where $I(.)$ is an indicator function that returns $1$ if the argument inside it is true and $0$ otherwise, $y_i$ refers to the true ideology of user $i$, $\hat{y_i}$ refers to the predicted ideology of user $i$ given by our model. Consequently, accuracy represents the proportion of users in a test set whose ideology is correctly classified by our model. 

\subsection{ROC-AUC}
\label{Methodology-model-assessment-auc}

To calculate the OVR ROC curves for a multi-class classification model's predictions on our test set we need, for each class $k$ ($k = 0,\dots,K-1$) and for each member of our test set, $i$, estimates of the probability that person $i$'s ideology is $k$: $\hat{P}(y_i = k)$. Then, for a set of thresholds, $\tau \in [0,1]$, we assign observation $i$ to $k$ if $\hat{P}(y_i = k) > \tau$ and to `not $k$' otherwise. We then compute the sensitivity (true positive rate) and $1-$specificity (specificity is the true negative rate):

$$ \text{sensitivity} = \cfrac{\text{TP}}{\text{TP + FN}} =
\cfrac{\sum_{y_i = k}I(\hat{P}(y_i = k) > \tau)}
{\sum_{i=1}^n I(y_i = k)
}$$
$$ \text{specificity} = \cfrac{\text{TN}}{\text{FP + TN}} =
\cfrac{\sum_{y_i \not = k} I(\hat{P}(y_i \le \tau))}
{\sum_{i=1}^n I(y_i \not = k)}$$

We plot the values for sensitivity and $1-$specificity in $\langle \text{1-specificity, sensitivity} \rangle$ space for each $\tau$. The area under this curve is the ROC-AUC for class $k$; $\text{roc auc}_k$. We compute the AUC for each class and weight it by the total proportion of testing observations in class $k$; $p_k$. We sum these $K$ weighted, class specific ROC-AUC values to gain an overall testing ROC-AUC estimate for our model\cite{989510}:

$$ \text{roc auc} = \sum^K_{k=1} \text{roc auc}_k \cdot p_k $$

The OVR ROC-AUC for class $k$ is equivalent to the probability that the classifier will assign a randomly selected observation from class $k$ a higher probability of membership in class $k$ than a randomly selected observation from some class other than $k$\cite{989510}. Thus, it is essentially a measure of how well our classifier can distinguish between classes, weighted by class prevalence. This method of averaging OVR ROC-AUC scores is referred to as the `weighted' method in SciKit-Learn\cite{scikit-learn}.

For binary classification problems we simply compute the probability that each observation belongs to one of the two classes (left/right or auth/lib) and compute the sensitivity and $1-\text{specificity}$ associated with varying thresholds to construct the ROC curve and therefore determine ROC-AUC.

ROC curves can only be constructed for models that can estimate the probability that an observation belongs to a class. As such, we omit the ROC-AUC metric from the evaluation of some models. Exactly how probability estimates are obtained from each model can be seen in the Scikit-Learn documentation\cite{scikit-learn}.


\section{Overview of statistical learning approaches}
\label{Methodology-overview-stat-learning}

\subsection{Singular value decomposition}
\label{Methodology-svd}

Singular value decomposition (SVD) is a dimension reduction technique that allows us to replace our data matrix, $X_{(n \times p)}$, with a lower-dimensional representation: a matrix $\bar{X}_{(n \times q)}$ where $q < p$. The SVD computation finds the $p$-dimensional vector, $\vec{v_1}$, in feature space that minimises the projection error of data onto the vector. This is the first SVD component. We can then represent each data point by its projection onto this vector. The distribution of the projected values of data points has the largest variance of any possible projection. We then determine subsequent SVD components by finding the $p$-dimensional vectors that maximise the variance of projected data points subject to the constraint that the vectors are orthogonal to existing SVD components. We do this until we have $q$ vectors.

Mathematically, we are decomposing the data matrix, $X$, into the product of three matrices: 

$$ X_{(n \times p)} = U_{(n \times r)} \Sigma_{(r \times r)} V^{\intercal} _{(r \times p)}$$

Here, $U$ is an $n \times r$ matrix where the $n$ rows correspond to users and the $r$ columns correspond to `themes' in the subreddit interaction data; i.e. latent factors. Any particular cell $u_{(i,\,j)}$ intuitively represents how much user $i$ interacts with theme $j$. $\Sigma$ is a $(r \times r)$ diagonal matrix where  $\sigma_{(i,\,i)}$ represents the variance of theme $i$. $V$ is a $(p \times r)$ matrix that, when transposed, maps interaction with subreddits to themes, i.e. $v^{\intercal} _{(i,\,j)}$ represents how much each interaction with subreddit $j$ adds or detracts from the the score on theme $i$. $\vec{v_q}$ is the $q_{th}$ row of the matrix $V^{\intercal}$.

We chose to use the first 500 SVD components as features in the relevant models. In conjunction with trimming, this reduced the amount of features in the user-interaction matrix from over 190,000 to 500. This accounts for roughly $86\%$ of the variance of the original data. 

As noted by Kosinski et al., principal component analysis (PCA) is a less appropriate technique for the kind of problem we are dealing with. PCA requires that the data be centered which does not preserve sparsity and therefore undermines efficient computation\cite{Kosinski2016MiningBD}.

\subsection{OVR logistic regression}
\label{Methodology-ovr-logreg}

We first describe a simple logistic regression (as used in our binary classification problems) and then explain how it can be extended to use in multi-class classification problems through a OVR scheme. 

A logistic regression models assumes that, when individual $i$ makes the binary decision $y_i \in \{ 0,\: 1\}$, the probability they choose $y_i=1$ is given by:

$$ P(y_i = 1|x_i;\,\beta) = \cfrac{e^{x_i^{\intercal} \beta}}{1+e^{x_i ^{\intercal} \beta}}$$

Where $x_i$ is a vector of predictors (often 500 SVD components in our case) with $x_{i, 0} = 1$ to allow for a constant term. $\beta = (\beta_0,  \beta_1, \dots, \beta_{500})^{\intercal}$ is a vector of coefficients to be estimated. Estimated model coefficients, $\hat{\beta}$, are obtained via maximum likelihood estimation (MLE), i.e. through solving the following maximization problem\cite{10.5555/2834535} (where $i = 1,\dots,n$ now indexes observations in our training set):

$$ \hat{\beta} = \underset{\beta}{\mathrm{argmax}} \left\{ 
\frac{1}{n} \sum^n_{i=1} w_i \{ 
y_i \ln P(y_i = 1|x_i;\,\beta) + (1-y_i) \ln (1 - P(y_i = 1|x_i;\,\beta) )
\}
\right\}$$

$w_i$ is the weight for each observation. We try both a uniform weighting and balanced weighting: $w_i = \frac{n}{n_i}$  where $n_i$ refers to the number of observations in the same class as observation $i$. 

With our MLE estimate of $\beta$, $\hat{\beta}$, we can can estimate the probability that some person $j$, who does not feature in our training set, chooses $y_j=1$ as:

$$ \hat{P}(y_j = 1|x_i; \, \hat{\beta}) = \cfrac{e^{x_j^{\intercal} \hat{\beta}}}{1+e^{x_j ^{\intercal} \hat{\beta}}} $$

This works for binary dependent variables but we are often attempting to classify ideologies where our dependent variable, $y_i$, takes on one of the following forms:

\begin{itemize}
    \item $y_i \in \{\text{libleft, libright, libcenter, centrist, left, right, authright, authleft}\}$
    \item $y_i \in \{\text{left, center, right}\}$
    \item $y_i \in \{\text{authoritarian, center, libertarian}\}$
\end{itemize}

We can extend the binary model using a technique called OVR logistic regression which involves fitting a model for each class to predict the probability that someone is in that class versus not in that class.

Consider the economic ideology classification problem where $y_i \in \{\text{left, center, right}\}$. The OVR logistic regression approach to modelling this problem involves fitting three different logistic regression models ($\beta,\, \gamma,\text{ and } \delta$ are all separate coefficient vectors to be estimated, MLE estimates are denoted by $\hat{\beta},\, \hat{\gamma},\text{ and } \hat{\delta}$). 

\textbf{Model 1 - predict probability that individual is left versus not left:}

$$ \hat{P_1}(y_i = \text{left}|x_i;\,\hat{\beta}) = \cfrac{e^{x_j^{\intercal} \hat{\beta}}}{1+e^{x_j ^{\intercal} \hat{\beta}}} $$

\textbf{Model 2 - predict probability that individual is center versus not center:} 

$$ \hat{P_2}(y_i = \text{center}|x_i;\,\hat{\gamma}) = \cfrac{e^{x_j^{\intercal} \hat{\gamma}}}{1+e^{x_j ^{\intercal} \hat{\gamma}}} $$

\textbf{Model 3 - predict probability that individual is right versus not right:}

$$ \hat{P_3}(y_i = \text{right}|x_i;\,\hat{\delta}) = \cfrac{e^{x_j^{\intercal} \hat{\delta}}}{1+e^{x_j ^{\intercal} \hat{\delta}}} $$

We assign individual $j$ to the class for which the relevant OVR probability expression is largest. For example, we assign $j$ to left iff:

$$ \cfrac{e^{x_j^{\intercal} \hat{\beta}}}{1+e^{x_j ^{\intercal} \hat{\beta}}} > 
\cfrac{e^{x_j^{\intercal} \hat{\gamma}}}{1+e^{x_j ^{\intercal} \hat{\gamma}}}, \text{ and }
\cfrac{e^{x_j^{\intercal} \hat{\beta}}}{1+e^{x_j ^{\intercal} \hat{\beta}}} > 
\cfrac{e^{x_j^{\intercal} \hat{\delta}}}{1+e^{x_j ^{\intercal} \hat{\delta}}}$$

\subsection{OVR logistic regression with \texorpdfstring{$\ell_1$}{Lg} penalty}
\label{Methodology-ovr-logreg-l1}

To improve upon the basic logistic regression model, we can augment the log likelihood by subtracting (a proportion of) the $\ell_1$ norm of the coefficient vector from the log likelihood. Thus, we obtain coefficient estimates through solving the following maximization problem:

$$ \hat{\beta} = \underset{\beta}{\mathrm{argmax}} \left\{ 
\frac{1}{n} \sum^n_{i=1} w_i \{ 
y_i \ln P(y_i = 1|x_i;\,\beta) + (1-y_i) \ln (1 - P(y_i = 1|x_i;\,\beta) )
\} - \lambda ||\beta_{/0}||_1 \}
\right\}$$

Where $\lambda > 0$ and $||\beta_{/0}||_1$ refers to the $\ell_1$ norm of the $(p \times 1)$ vector $\beta_{/0}$, which is the vector of coefficients associated with all regressors excluding  the intercept term. i.e. $||\beta_{/0}||_1 = \sum^p_{j=1} |\beta_j|$.  

When coefficients deviate from zero in magnitude, $\lambda ||\beta_{/0}||_1$ increases, thus penalising the augmented log-likelihood. This has the effect of shrinking unimportant coefficients to zero and may improve predictive accuracy if the decrease in model variance more than offsets the increase in model bias\cite{10.5555/2517747}. The lasso penalty can be viewed as the imposition of a constraint on the size of parameters onto the maximisation problem discussed in Section \ref{Methodology-ovr-logreg}. The parameter $\lambda$ is a tuning parameter that controls the strength of the regularization; a higher $\lambda$ implies stronger regularization i.e. a smaller budget for the maximum $\ell_1$ norm of the coefficient vector. 

This process provides a different set of coefficient estimates (with many possibly being equal to zero, effectively dropping irrelevant features from the model) but the process of prediction and implementation of the OVR scheme is the same as in Section \ref{Methodology-ovr-logreg}.

\subsection{Multinomial logistic regression}
\label{Methodology-multinomial}

Multinomial logistic regression is an extension of logistic regression that can naturally perform multi-class classification. When there are $K$ choices ($k = 0,\dots,K-1$), the probability that individual $i$ chooses choice $k$ is given by:

$$P(y_i = k |x_i,\; \beta_k) = \begin{cases}
\cfrac{1}{1+\sum^K_{k\prime=1} e^{x_i ^{\intercal} \beta_{k\prime}}} & k = 0,\\
\cfrac{e^{x_i ^{\intercal} \beta_k}}{1+\sum^K_{k\prime=1} e^{x_i ^{\intercal} \beta_{k\prime}}} & k \not = 0 
\end{cases}$$

Thus, prediction requires the estimation of a separate coefficient vector $\beta_k$ for each class. By convention, $\beta_0$ is set to $\vec{0}$ since we cannot uniquely identify any particular $\beta_k$, we can only identify $(\beta_k - \beta_0)$\cite{10.5555/2834535}. 

Coefficient vector estimates, $\hat{\beta}_1,\dots,\hat{\beta}_{K-1}$,  are found by solving the following maximization problem:

$$ \hat{\beta}_1,\dots,\hat{\beta}_{K-1} = \underset{\beta_1,\dots,\beta_{K-1}}{\mathrm{argmax}} \left\{ \frac{1}{n}\sum^n_{i=1} w_i \sum^K_{k=1} I(y_i = k) \ln P(y_i = k | \beta_k) \right\} $$ 

This allows us to compute the predicted probability that a new observation, $j$, belongs to any particular class like so: 

$$\hat{P}(y_i = k | x_i;\;\hat{\beta}_k) = \begin{cases}
\cfrac{1}{1+\sum^K_{k\prime=1} e^{x_i ^{\intercal} \hat{\beta}_{k\prime}}} & k = 0,\\
\cfrac{e^{x_i ^{\intercal} \hat{\beta}_k}}{1+\sum^K_{k\prime=1} e^{x_i ^{\intercal} \hat{\beta}_{k\prime}}} & k \not = 0 
\end{cases}$$

We assign $j$ to $\underset{k}{\mathrm{argmax}}\, \hat{P}(y_j = k|\hat{\beta}_k)$ to obtain a categorical prediction.

\subsection{Multinomial logistic regression with \texorpdfstring{$\ell_1$}{Lg} penalty}
\label{Methodology-multinomial-l1}

The $\ell_1$ penalty described in Section \ref{Methodology-ovr-logreg-l1} can also be fruitfully applied to multinomial logistic regression. Thus, we are choosing $\hat{\beta}_1,\dots,\hat{\beta}_{K-1}$ to maximise\cite{10.5555/2834535}:

$$ \hat{\beta}_1,\dots,\hat{\beta}_{K-1} = \underset{\beta_1,\dots,\beta_{K-1}}{\mathrm{argmax}} \left\{ \frac{1}{n}\sum^n_{i=1} w_i \sum^K_{k=1} I(y_i = k) \ln P(y_i = k | \beta_k)  - \lambda \sum^K_{k=1} ||\beta_{k,/0}||_1 \right\}$$ 

Where $\beta_{k,/0}$ refers to the coefficient vector $\beta_k$ without the intercept coefficient. 

This has the same effect as described in Section \ref{Methodology-ovr-logreg-l1}\cite{10.5555/2834535}. The rest of the classification procedure after model estimation is the same as described in Section \ref{Methodology-multinomial}.

\subsection{OVR linear support vector classifier}
\label{Methodology-svc}

We describe a linear support vector classifier (SVC) for a binary classification problem. This is extended to multi-class classification via a OVR scheme that determines an observation's class on the basis of its distance between several, class specific separating hyperplanes. 

The SVC estimates a linear decision boundary in feature space by finding the hyperplane that maximises the margin (euclidean distance between the hyperplane and the observations closest to the hyperplane from either class) subject to a certain tolerance for training observations that violate the margin (i.e. that are on the `wrong' side of the margin). 

The coefficients for this hyperplane, $\hat{\beta}= (\hat{\beta}_0, \hat{\beta}_{/0}^{\intercal})^{\intercal}$ are found by solving the following problem\cite{10.5555/2517747}:

$$
\hat{\beta} = 
\underset{\beta}{\mathrm{argmin}} =
\cfrac{1}{2} \beta_{/0}^\intercal \beta_{/0} + C
\sum_{i=1}^n \max(0,\, y_i(\beta_{/0}^\intercal x_i + \beta_0))$$


Here $x_i$ does not include a constant first element equal to one. $C$ is a constant that is \textit{inversely} proportional to the strength of regularization\footnote{In some formulations of the linear SVC maximization problem C refers to the regularization parameter itself but we follow the formulation given in the Scikit-Learn documentation.}. Higher values of $C$ will correspond to a stricter margin with less tolerance for violation.

We can predict the class of an observation, $j$, depending on which side of the estimated separating hyperplane it falls, i.e depending on the sign of $x_j^{\intercal}\hat{\beta}$.

\subsection{Term frequency - inverse document frequency}
\label{Methodology-tfidf}

The first step in this process of feature extraction is to `clean' the text. We remove all html links, punctuation, non ascii symbols (i.e. emojis) and single letter terms, convert all terms to lower case, and finally stem all terms. 

Then, for each word, $w$, we compute the `term frequency' for user $i$:

$$TF_{w,i} = \cfrac{n_{w,i}}{\sum_{k=1}^{K} n_{k,i} }$$

Where $n_{w,i}$ refers to how many times word $w$ appears in user $i$'s concatenated comments and $k=1,\dots,K$ indexes all words appearing in our vocabulary of terms (which is defined by the terms in the total set of all comments).

We then compute the inverse document frequency (IDF) of each word\footnote{This specific form is implemented by our models and differs slightly from standard textbook definitions of inverse document frequency.}:

$$IDF_w = \ln \left( \cfrac{D+1}{D_w+1}\right)  + 1$$

Where $D$ refers to the total number of users whose comments we have recorded (total amount of documents) and $D_w$ is the amount of concatenated sets of comments containing word $w$. 

Consequently, $TF_{w,i}\cdot IDF_w$ measures how much user $i$ uses word $w$ relative to other users. We construct the inverse document frequency for every word in our training vocabulary that has not been excluded by some criteria and then create tf-idf scores for each user (both in the training and testing set) for all of these terms. We then normalise tf-idf vectors for each user by their euclidean norm. 

Several hyperparameters impact the set of terms for which we compute tf-idfs, namely the maximum and minimum frequency of words which we allow in our vocabulary. Words that occur in a greater proportion of documents than our maximum frequency or in a smaller proportion of documents than our minimum frequency are disregarded. We also specify the maximum amount of words in the vocabulary, where words are ranked according to their term frequency across the corpus.

\subsection{Word2Vec}
\label{Methodology-embed}

Word2Vec is an unsupervised learning algorithm that takes a corpus of text and `learns' to represent each word as a vector. We use embedding from a model that has been pre-trained  on Google News data. This model contains 300-dimensional vectors for around 100,000,000,000 words and does not require that we convert our text to lower case or remove punctuation. Using a pre-trained model allows us to avoid training our own model which is time consuming and may be inaccurate due to our relatively small corpus.

The workings of the Word2Vec algorithm are somewhat complex so for the sake of brevity we refer the reader to \cite{Mikolov2013} and \cite{Mikolov2013a}.




==> Chapter5.tex <==
\chapter{Results}
\label{Results}

\section{Model results}
\label{Results-model}

The accuracy and ROC-AUC (where applicable) of every model estimated for all binary and three-class models can be found in \tref{table.results_1}

\begin{table}[!htbp] %htbp
  \centering
  \caption{Binary and multi-class classification of economic and social ideology \\ 
\scriptsize  N refers to the total amount of samples divided between training, validation and testing sets. In the multi-class problem AUC refers to weighted ROC-AUC}
      \scalebox{0.70}{
    \begin{tabular}{lllllllll}
    \makebox[0pt][l]{\textbf{Binary economic classification}} &       &       &       &       & \makebox[0pt][l]{\textbf{Binary social classification}} &       &       &  \\
    Model & Accuracy & AUC   & N     &       & Model & Accuracy & AUC   & N \\
\cmidrule{1-4}\cmidrule{6-9}    \makebox[0pt][l]{\textit{Features: user-interaction matrix}} &       &       &       &       &       &       &       &  \\
\cmidrule{1-4}\cmidrule{6-9}    ZeroR & 56.06\% &       & 52,881 &       & ZeroR & 78.99\% &       & 54,151 \\
    Random forest & 73.38\% & 81.29\% & 52,881 &       & Random forest & 80.47\% & 72.63\% & 54,151 \\
    AdaBoost & 79.07\% & 87.76\% & 52,881 &       & AdaBoost & 81.29\% & 73.98\% & 54,151 \\
    Logit ($\ell_1$) & 82.37\% & 90.63\% & 52,881 &       & Logit($\ell_1$) & 82.00\% & 78.66\% & 54,151 \\
    Logit  & 82.38\% & 90.63\% & 52,881 &       & Logit  & 82.02\% & 78.66\% & 54151 \\
          &       &       &       &       &       &       &       &  \\
    \makebox[0pt][l]{\textit{Features: textual features}} &       &       &       &       &       &       &       &  \\
\cmidrule{1-4}\cmidrule{6-9}    ZeroR & 54.07\% &       & 57,045 &       & ZeroR & 76.62\% &       & 59,055 \\
    Linear SVC; w2v & 66.68\% &       & 57,045 &       & Linear SVC; w2v & 76.62\% &       & 59,055 \\
    Linear SVC; tf-idf & 72.57\% &       & 57,045 &       & Linear SVC; combined & 79.94\% &       & 59,055 \\
    Linear SVC; combined & 73.21\% &       & 57,045 &       & Linear SVC; tf-idf & 79.98\% &       & 59,055 \\
          &       &       &       &       &       &       &       &  \\
    \makebox[0pt][l]{\textit{Features: combined}} &       &       &       &       &       &       &       &  \\
\cmidrule{1-4}\cmidrule{6-9}    ZeroR & 56.06\% &       & 51,199 &       & ZeroR & 79.42\% &       & 52,399 \\
    Logit ($\ell_1$) & 82.29\% & 90.38\% & 51,199 &       & Logit ($\ell_1$) & 82.69\% & 79.12\% & 52,399 \\
    Linear SVC & 82.83\% &       & 51,199 &       & Linear SVC & 83.09\% &       & 52,399 \\

  & &  &  & & &  &  & \\
 
    \makebox[0pt][l]{\textbf{Multi-class economic classification}} &       &       &       &       & \makebox[0pt][l]{\textbf{Multi-class social classification}} &       &       &  \\
\cmidrule{1-4}\cmidrule{6-9}    \makebox[0pt][l]{\textit{Features: user int}} &       &       &       &       &       &       &       &  \\
\cmidrule{1-4}\cmidrule{6-9}    ZeroR & 36.63\% &       & 80,961 &       & Multinomial logit ($\ell_1$) & 48.16\% & 66.68\% & 80,961 \\
    OVR Random Forest & 51.10\% & 69.68\% & 80,961 &       & ZeroR & 52.84\% &       & 80,961 \\
    Random forest & 51.13\% & 70.79\% & 80,961 &       & Random forest & 53.93\% & 62.58\% & 80,961 \\
    AdaBoost & 53.69\% & 72.03\% & 80,961 &       & OVR Random Forest & 53.98\% & 63.72\% & 80,961 \\
    OVR Logit  & 57.36\% & 76.43\% & 80,961 &       & AdaBoost & 54.00\% & 63.21\% & 80,961 \\
    Multinomial logit ($\ell_1$) & 57.50\% & 76.59\% & 80,961 &       & Multinomial logit & 55.82\% & 67.35\% & 80,961 \\
    Multinomial logit & 57.52\% & 76.54\% & 80,961 &       & OVR Logit  & 55.94\% & 67.31\% & 80,961 \\
    OVR Logit ($\ell_1$) & 57.65\% & 76.51\% & 80,961 &       & OVR Logit ($\ell_1$) & 55.94\% & 67.31\% & 80,961 \\
          &       &       &       &       &       &       &       &  \\
    \makebox[0pt][l]{\textit{Features: textual features}} &       &       &       &       &       &       &       &  \\
\cmidrule{1-4}\cmidrule{6-9}    ZeroR & 35.07\% &       & 87,547 &       & ZeroR & 51.40\% &       & 87,547 \\
    Linear SVC; w2v & 41.56\% &       & 87,547 &       & Linear SVC; w2v & 51.91\% &       & 87,547 \\
    Linear SVC; tf-idf & 48.94\% &       & 87,547 &       & Linear SVC; combined & 53.14\% &       & 87,547 \\
    Linear SVC; combined & 49.00\% &       & 87,547 &       & Linear SVC; tf-idf & 53.71\% &       & 87,547 \\
          &       &       &       &       &       &       &       &  \\
    \makebox[0pt][l]{\textit{Features: combined}} &       &       &       &       &       &       &       &  \\
\cmidrule{1-4}\cmidrule{6-9}    ZeroR & 36.83\% &       & 78,348 &       & ZeroR & 53.22\% &       & 78,348 \\
    OVR Logit ($\ell_1$) & 57.31\% & 76.46\% & 78,348 &       & OVR Logit ($\ell_1$) & 56.28\% & 67.17\% & 78,348 \\
    Linear SVC & 57.63\% &       & 78,348 &       & Linear SVC & 56.56\% &       & 78,348 \\
    \end{tabular}}
  \label{table.results_1}%
\end{table}%

In the binary classification of economic ideology ($y_i \in \{ \text{left, right} \}$) using only the user-interaction matrix as features, our best model\footnote{Best model refers to the model with the highest testing accuracy.}, logistic regression's, predictions on the test set achieved an accuracy of 82.38 \% (against a ZeroR baseline of 56.06 \%) and an ROC-AUC of 90.63\%. This reinforces Kosinski et al’s findings. Kosinski et al. were able to predict whether a Facebook user was a Democrat or Republican based off their Facebook Likes\cite{kosinski2013private} (noting that they do not omit Facebook Likes for explicitly political pages) with an ROC-AUC of 85\%.   

In contrast, our best model in the binary classification of social ideology ($y_i \in \{ \text{lib, auth}\}$) using only the user-interaction matrix, logistic regression, barely improved upon the ZeroR baseline accuracy of 78.99\%, achieving an accuracy of 82.02\% on testing data. The model achieved an ROC-AUC of 78.66\% on the test set\footnote{The high ROC-AUC figure here cannot be trusted as the response variable is highly imbalanced as indicated by the ZeroR classification accuracy.}.

Textual features were worse performers in the binary classification problems. In predicting economic ideology, the linear SVC applied to the union of tf-idf features and average Word2Vec features (which was the best model in this task) achieved an accuracy of 73.21\% relative to the 54.07\% ZeroR baseline. For social ideology, the best model, a linear SVC using just tf-idf features, achieved an accuracy of 79.98\% against a 76.62\%  baseline\footnote{ZeroR baselines slightly differ between models due to different splits.}. Interestingly, this illustrates that the difficulty of predicting social ideology relative to economic ideology is robust to the type of digital record employed. 

The models that utilised both the user-interaction matrix and textual footprints (tf-idf features) did not substantially improve upon the performance of the models that solely used the user-interaction matrix as features. 

We now report the performance of models in the economic and social ideology classification tasks when we did not omit centrist observations, i.e. when we classify $y_i \in \{ \text{left, center, right} \}$ and $y_i \in \{ \text{lib, center, auth}\}$. Using just the user-interaction matrix, in the economic classification task our best model, OVR logistic regression with an $\ell_1$ penalty, achieved an accuracy of 57.65\% against a ZeroR baseline of 36.63\% and an ROC-AUC of 76.51\%. For the social problem, OVR logistic regression marginally surpassed baseline performance, achieving an accuracy of 55.94\% (baseline: 52.84\%) and an ROC-AUC of 67.31\%.

The models using textual features again perform worse than those using the user-interaction matrix. The best economic classifier using textual features (linear SVC using a union of tf-idf features and average Word2Vec features) still performs substantially better than baseline benchmarks (accuracy: 49.00\% vs 35.07\% ZeroR accuracy). The best social classification model (linear SVC using just tf-idf features) achieves an accuracy of 53.71\% against a 51.40\% baseline. This indicates that the classification of economic ideology is robust to the inclusion of centrists (i.e. we can still classify users’ ideology  at an accuracy substantially above baseline), albeit with significantly diminished accuracy. We also see that the stronger performance of the user-interaction matrix relative to textual features is robust to the inclusion of centrists. 

We suspect the primary reason for the comparatively poor performance of textual features is the limited variation in language use in our sample. The r/PoliticalCompassMemes subreddit is an online subculture with its own vernacular. For instance, many users of all ideologies use jargon such as `based’ and `cringe’ to indicate appreciation or dissatisfaction. We scraped comments from subreddits outside of r/PoliticalCompassMemes to try and maximise variation in word use but the use of the vernacular likely persists in other subreddits. Further, though we are unable to rigorously validate this claim, most users are likely young; many users in our sample comment in subreddits indicative of age, i.e. r/teenagers and appear to be located in the United States based on the prevalence of discussion topics relevant to US politics.

This effectively restricts the variation in vocabulary used by r/PoliticalCompassMemes commentors making it harder to link variation in language to ideology. The lack of variation in language is shown in \fref{fig.word_freq} (the frequency of the n-word and `cum' is due to a handful of `troll' users who have made many comments which repeat these words thousands of times).

\begin{figure}[!htbp]
\centering
  \fbox{\includegraphics[width=14cm,height=8.75cm]{Figures/word_freq.pdf}}
  \caption{Word frequencies in comments by ideology \label{fig.word_freq}}
\end{figure}


Still, variation in language is associated with ideology and textual features remain useful. To provide some insight into which facets of language are most associated with ideology we display the words most strongly correlated with economic and social ideologies in \fref{fig.wordcloud}.

\begin{figure}[!htbp]
\centering
  \fbox{\includegraphics[width=14cm,height=14cm]{Figures/wordclouds.pdf}}%
  \caption{Economic ideology was recoded from \{left, center, right\} to \{-1, 0, 1\} and social from \{lib, center, auth\} to \{-1, 0, 1\}. We then computed the correlation of the tf-idf scores for each term with the quantitative ideology measure. Size of terms in wordclouds is proportional to correlation with the relevant ideology 
  \label{fig.wordcloud}}
\end{figure}

Again, in the multi-class classification problems, the union of the user-interaction matrix and textual features does not lead to models with substantively better performance on unseen data. We suspect that this is due to colinearity between the user-interaction features and textual features. In the same way that r/PoliticalCompassMemes has its own vernacular, interaction with  subreddits is likely associated with particular language usage. If a user has made comments in the r/Vegetarian subreddit then they have likely used language strongly associated with  vegetarianism, i.e. `vegan’, `meat’, `dairy’, increasing the value of textual features associated with use of these words. Thus, engagement with subreddits and language use likely go hand in hand in many cases and there is little information gained from textual features when we have already employed records of subreddit interaction. 

The final set of models estimated predict which of the full nine classes each user belongs to, i.e. $y_i \in \{ \text{centrist, left, right, libright, libleft, libcenter, authright, authleft, authcenter}\}$. Understandably, these models feature the lowest accuracy due to the abundance of possible classes. Nevertheless, the best model based on the user-interaction matrix (multinomial logistic regression) was able to substantially improve upon baseline accuracy achieving an accuracy of 34.82\% against the 20.81\% ZeroR baseline and an AUC of 74.61\%. The best nine-class classification model using solely textual data (linear SVC on the union of tf-idf features and average Word2Vec features) performs worse than the best model using solely interaction data, achieving an accuracy of 24.4\% against the 19.84\% ZeroR baseline. The union of textual features with the user-interaction matrix does not substantially improve performance in the nine-class classification problem. \tref{table.results_2}, which provides the full set of results for all models in the nine-class problem, has been relegated to Appendix \ref{Appendix-nineclass} as these results are somewhat ancillary to our other findings. 

\section{Insights}
\label{Results-viz}

In \fref{fig.int_eda} we display the proportion of total comments from each ideology in  particular subreddits. This is intended to illustrate the variation in subreddit interaction between users of different ideologies and how Reddit data can illuminate psycho-social dynamics. From  the first row, one could infer that those with more left-leaning economic views are more comfortable discussing any mental illnesses they are facing. This also illustrates how digital footprints related to mental health (i.e. search engine queries relating to a condition) are the type of digital footprint that could provide information on a person's political beliefs despite the fact there is no obvious connection between mental health and political ideology.   

\begin{figure}[!htbp]
\centering
  \fbox{\includegraphics[width=14cm,height=17.5cm]{Figures/interactions_eda.pdf}}%
  \caption{This figure shows the proportion of total comments from users of each ideology in a range of subreddits  \label{fig.int_eda}}
\end{figure}

The second row of \fref{fig.int_eda} illustrates how libertarian users of any economic persuasion (but especially those with right wing economic views) interact the most with r/Bitcoin. This makes sense as Bitcoin is a decentralised digital currency that can be used anonymously; which would naturally appeal to those who are skeptical of state power and value political freedom highly. We also see that economically right wing users interact most with the popular r/wallstreetbets subreddit which is focused on risky trading strategies in financial markets. Economically right wing users also interact more with the r/conspiracy subreddit. 

The third row of \fref{fig.int_eda} shows these results for several subreddits that common wisdom dictates would be favoured by users with progressive views. r/lgbt is a subreddit for people with sexual orientations other than heterosexual, r/AgainstHateSubreddits is a forum focused on identifying and denouncing other subreddits perceived to have engaged in prejudiced behaviour and r/TwoXChromosomes is a subreddit for women (studies show women tend to lean further left). Variation in the amount of interaction with these subreddits along ideological lines allows for digital footprints to predict ideology\footnote{Right wing authoritarian users have the largest proportion of comments/posts in r/AgainstHateSubreddits which is contrary to expectation. A brief investigation suggests that this may be because users from r/AgainstHateSubreddits have targeted r/PoliticalCompassMemes due to the posts of the more conservative users. Consequently, some conservative users comment in r/AgainstHateSubreddits to engage in argument.}.  

Of greater concern is the fact that interactions with subreddits that do not pertain to politically charged interests exhibit substantial variation with respect to ideology. For example, as illustrated in the final row, those with authoritarian views seem to have much less interest in movies, video games or sport; perhaps those with authoritarian views are more committed to their political beliefs and consequently these beliefs form a larger part of their identity leaving them less interested in non-political activities. The upshot here is that digital footprints indicating something as simple as your interest in movies or sports are informative with respect to ideology. 

Returning now to textual footprints, in \fref{fig.wordcloud} we see some expected results, right wing economic ideology (which is likely correlated with right wing social views) is correlated with frequent talk of guns, taxes and similar topics. There are also some more subtle results which reflect the psychological basis of ideology. We see that right wing views are correlated with using words like “theft”, “felon” and “defence”, a reflection of the fact that conservatives tend to have a larger fear of threat and loss\cite{Jost2007}. We also see words like “degenerate” and “whore” which picks up on the higher disgust sensitivity of conservatives\cite{Inbar2011}. Contrastingly, when it comes to left wing economic views, we see many words related to sexuality indicating a much more open discourse on these topics, perhaps linked with lower disgust sensitivity. Concerningly, words with no obvious political connotations correlate just as much as  explicitly political language. `Specific’ appears to correlate with left wing views as strongly as ‘proletariat’ and ‘cute’ as much as ‘queer’. Words indicating ambiguity (`maybe', `sometimes', `confused') and terms related to music (`album', `song') also appear as top linguistic correlates of left wing economic views. This is a frightening reminder of how digital footprints of an entirely non-political nature can be leveraged to infer ideology.


\newpage

==> Chapter6.tex <==
\chapter{Discussion}
\label{Discussion}


We have shown that, publicly available, largely non-political digital footprints can be mapped to ideology with greater than baseline accuracy. This broader claim provides validation of existing results but we have also made several novel contributions: 

\begin{enumerate}
    \item Showing that digital footprints are able to predict the economic dimension of ideology to a high degree of accuracy even in a multi-class classification problem that includes centrists, although this is a trickier, noisier problem than binary ideological classification. 
    \item Showing that digital footprints are better predictors of economic ideology than social ideology.
    \item Showing that textual data is less predictive of ideology than interactions data.
\end{enumerate}

The first two points have important policy upshots, though we only discuss the first point for the sake of brevity. We do not believe the third point should inform policy as this finding appears to be due to an idiosyncratic feature of our data as detailed in Section \ref{Results-model}.

\section{Policy implications}
\label{Discussion-policy}

Our results show that digital footprints can predict ideology in a nine-class problem where ideology is a complex variable that contains both an economic and social element. We also show that we can predict economic ideology above baseline accuracy when we account for the existence of centrists, but our predictions are far better when we omit centrists. In general, the more classes we include, the poorer our classifiers performed.  

Consider an (for the sake of discussion, right wing party's) election strategist with access to digital footprints from a broad range of voters as well as a model that maps these footprints to ideology. This strategist would likely want to know as much about each voter's ideology as possible. They might wish to emphasise their party's candidate's libertarian economic policy to the `libertarian right' voters whilst emphasizing their candidate's `tough on crime' policies to `authoritarian right' voters and target economically left leaning voters with advertisement designed to discourage them to vote. That is to say, they want a model that can accurately assign each voter to one of many ideological classes. Our results indicate that such a model might be hard to develop.

In contrast, an authoritarian government may want a model that can differentiate the majority of those with conforming ideologies from those with dissenting views. Our results indicate that this is a much more plausible task; models work best when separating two disparate ideologies with the absence of `noisy' ideologies, i.e. those occupying the middle-ground between two extremes. 

\section{Reddit's role in social data science}
\label{Discussion-reddits-role}

Our paper has further illustrated that data from Reddit can be fruitfully utilised in the social sciences. As mentioned, many prior studies in this area relied on Facebook data and linked digital footprints such as Facebook Likes with private traits. The fact that Facebook data is no longer easily accessible to researchers is naturally a poor outcome for this area of inquiry. However, by illustrating Reddit data to be a viable alternative for this sort of inquiry, we hope to revitalise this field. 

For instance, there are a broad range of Reddit communities where users reveal certain traits (whether through flairs or other means) that can be studied to examine the lins between traits and online behaviour, or traits and behaviour full stop (using online actions as a proxy for general behaviour, i.e. posting in drug related subreddits can be considered a proxy for drug use). 

Further, the data available from Reddit may be useful in other areas of social science research. For instance, using our data set, we could examine the connections between flaired ideology and participation in misogynistic online communities. These kinds of insights into the interactions between all sorts of social behaviours could inspire theories and experiments in a range of disciplines such as psychology, sociology and economics.

\section{Limitations}
\label{Discussion-Limitation}

One substantial limitation is that it is unclear how well our results generalise. Our data comes from  an online community for which the range of ages, interests and personality traits is likely narrower than in the general population. This issue is discussed extensively in Section \ref{Data-caveats}
so we do not repeat this exposition here for the sake of brevity. 

Another limitation is that our findings may underestimate the true extent to which digital footprints can predict ideology. The kinds of entities that are capable of misusing digital data in the ways we have discussed are governments and massive technology companies. Governments with sufficient surveillance capacity could, in principle, have access to every single digital footprint (Google searches, Facebook messages,  etc.) for each resident in their country from which they could develop powerful models. Tech companies also have a huge wealth of data on their users. In contrast, we are constrained to using publicly available information which we can scrape and manage on standard personal computers. Consequently, our results are perhaps an underestimate of the capabilities of the kinds of entities liable to estimate ideology from digital footprints with malignant intentions.  

Another limitation of this study pertains to the response variable. In studying the prediction of personal traits as a function of digital footprints, there is always a trade-off between the quality of the response variable and the sample size.  Studies that utilise a  sophisticated, scientific measure of ideology as their response variable will likely require volunteers to determine their ideology according to the measure and disclose their digital footprints. Such studies are, consequently, likely to feature a small sample size. Contrastingly, large samples of digital users can only be obtained by scraping publicly available digital records. Typically these records only contain snippets of information, such as party affiliation, or binary left/right ideological positioning rather than a complex, detailed picture of each user’s ideological beliefs. As explained, our ideological labels are substantially more sophisticated than those used in other studies with comparably large sample sizes. However, they are still far from perfect and provide a far less complete account of each users’ ideology than a measure such as the 12 Item Social and Economic Conservatism Scale\cite{Everett2013} would. Naturally, studies utilising more reliable and sophisticated measures of ideology are, ceteris paribus, more valuable and in an ideal world we would have a huge sample of users’s digital footprints alongside such measures. However, at present, it is hard to see how such data could be obtained. 

\section{Further research}
\label{Discussion-Further-research}

In this paper we used relatively simple predictive methods to map footprints to ideology. We showed that digital footprints can predict ideology but it is very possible that digital footprints can predict ideology with far greater accuracy than we have demonstrated. For instance, we used a singular value decomposition to reduce the dimensions of our data but did not experiment with other methods of dimension reduction, i.e. Uniform Manifold Approximation and Projection for Dimension Reduction\cite{McInnes2018}. Further, though our study uses a broader array of supervised learning algorithms than Kosinski et al.'s seminal paper\cite{kosinski2013private}, it could be rewarding to experiment with an even broader range of learning models. For instance, factorization machines look like a promising algorithm for this problem. Likewise, there are many other methods for extracting features from textual data that may be more easily mapped to ideology.  

In a similar vein, we could also extract different or additional features from our user-history records. In our user-interaction matrix, we extracted the number of times each user commented or posted in a particular subreddit. However, we could also extract the average (or total, maximum, minimum, etc.) score (`karma' in Reddit vernacular) of the users' posts/comments in each subreddit. Due to time constraints, we did not experiment with such an approach but these features could plausibly be used in conjunction with our existing user-interaction matrix to better predict ideology. 

Additionally, further contributions to this area could be made through a similar study with an expanded sample. Our sample size is larger than that of Kosinski et al.'s\cite{kosinski2013private},  however, we were still limited by time and resources. Our data was scraped over the course of several weeks using personal computers. With sufficient knowledge of scraping (to optimise the process) and greater resources and time, it would be possible to construct a much larger sample. It would be easier for learning algorithms to differentiate signal from noise in a larger sample which would be conducive to further refining our understanding of digital footprints' predictive power over ideology. Similarly, with sufficient  computational power to process more textual data, we could have collected more than (a maximum of) 100 comments per user.

\section{Ethics}

Our paper presents several ethical issues. Regarding the ethics of our data collection, the Reddit User Agreement states that users consent to having their comments publicly displayed on the internet and hence collectable by Reddit’s API.  Additionally, owing to the anonymity of the platform, none of the users whose data we have collected are at risk of physical, financial or reputational harm. 

It could be argued that this type of research facilitates the malignant use of the predictive technologies we have been developing. In response to any such claims we note that these predictive capabilities already exist and have widely been used in controversial applications (i.e. the Cambridge Analytica scandal). Our research is simply shining a light on this phenomena and further illuminating what is possible so that we may take action as necessary to counter the societal threats posed by such technology. Any entity seeking to abuse these capabilities would have no issue deploying similar predictive models without the aid of our paper. 

On that note, the ethics of deploying such technology will depend on the particular nature of the application. This is a complex topic that is beyond the scope of this thesis. 

==> Declaration.tex <==
% https://www.monash.edu/graduate-research/examination/publication
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis/writing-the-thesis-chapters/structuring-a-long-text
\Declaration{
\addtocontents{toc}{}  % Add a gap in the Contents, for aesthetics

This thesis is an original work of my research and contains no material which has been accepted for the award of any other degree or diploma at any university or equivalent institution and that, to the best of my knowledge and belief, this thesis contains no material previously published or written by another person, except where due reference is made in the text of the thesis.
\vfil\vfil\null
Signature:\\
\rule[1em]{25em}{0.5pt}  % This prints a line for the signature

Print Name: Xingbo Dong\\
\rule[1em]{25em}{0.5pt}  % This prints a line for the signature

Date:\\
\rule[1em]{25em}{0.5pt}  % This prints a line to write the date
}


==> Declaration_publications.tex <==
% https://www.monash.edu/graduate-research/examination/publication
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis/writing-the-thesis-chapters/structuring-a-long-text
\Declarationpublication{
\addtocontents{toc}{}  % Add a gap in the Contents, for aesthetics

\emph{This declaration is to be included in a `thesis including published works'. You must provide details of all publications included in your thesis in the section below. If you have not completed a thesis including published works.}

\emph{Please ensure your thesis meets the \href{https://www.monash.edu/graduate- esearch/examination/publication}{thesis including published works requirements}. Some faculties vary requirements in terms of the number of papers required, status of papers
and other criteria. These faculty specific requirements can also be found at the above link.}

\emph{Please remove the above section and include a standard thesis declaration.}

I hereby declare that this thesis contains no material which has been accepted for the award of any other degree or diploma at any university or equivalent institution and that, to the best of my knowledge and belief, this thesis contains no material previously published or written by another person, except where due reference is made in the text of the
thesis.

This thesis includes (\emph{insert number)} original papers published in peer reviewed journals and (\emph{insert number)} submitted publications. The core theme of the thesis is (\emph{insert theme}). The ideas, development and writing up of all the papers in the thesis were the principal responsibility of myself, the student, working within the
(\emph{insert name of academic unit}) under the  supervision of (\emph{insert name of supervisor}).

(The inclusion of co-authors reflects the fact that the work came from active collaboration between researchers and acknowledges input into
team-based research.) \emph{Remove this paragraph for theses with sole-authored work}

In the case of \emph{(insert chapter numbers}) my  contribution to the work involved the following:

\emph{(If this is a laboratory-based discipline, a paragraph outlining the assistance given during the experiments, the nature of the experiments and an attribution to the contributors could follow.})

Here should be the table!

I have / have not renumbered sections of submitted or published papers
in order to generate a consistent presentation within the thesis.

Student name:

Student signature: Date:

I hereby certify that the above declaration correctly reflects the
nature and extent of the student's and co-authors' contributions to this
work. In instances where I am not the responsible author I have
consulted with the responsible author to agree on the respective
contributions of the authors.

\textbf{Main Supervisor name:}

\textbf{Main Supervisor signature:} \textbf{Date:}


}

==> Publications.tex <==
% https://www.monash.edu/graduate-research/examination/publication
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis/writing-the-thesis-chapters/structuring-a-long-text
\Publicationslist{

\addtocontents{toc}{}  % Add a gap  \addtocontents{toc}{\vspace{1em}}  in the Contents, for aesthetics

You may wish to list your publications arising from your research degree enrolment using the standard citation format of your academic unit. Remove this section if you do not have publications.

Journal articles:

1) Dong, Xingbo, Zhe Jin, and Andrew Teoh Beng Jin. "A genetic algorithm enabled similarity-based attack on cancellable biometrics." 2019 IEEE 10th International Conference on Biometrics Theory, Applications and Systems (BTAS). IEEE, 2019.

2) xxx

}

==> Streamline.tex <==
\chapter{Introduction}
\label{Introduction}

Privacy concerns regarding online data have become increasingly prevalent in the wake of several high profile social media privacy scandals in recent years, most notably the Facebook-Cambridge Analytica data scandal\cite{CamAnalytica}. Of particular concern is the threat that we can inadvertently reveal private traits through seemingly innocuous online behaviour. This has serious real world implications. Consider the possibility of someone’s sexuality being accurately determined from records of their online behaviour. In countries with conservative attitudes towards sexuality, people with non-traditional sexual orientations would be at risk of having their sexuality exposed and being subject to prejudice and harm. 

Consequently, there is a growing body of academic work devoted to predicting the traits of individuals (personality, gender, sexuality, etc.) on the basis of their digital footprints. Understanding the extent to which such prediction is possible informs the appropriate level of concern that should be paid to matters of digital privacy policy. Existing work has largely focused on psychological (e.g. Big Five personality traits) and demographic traits (e.g. gender). For example, it has been shown that neural networks can accurately predict sexual orientation from pictures of an individual\cite{wang2018deep} and that Facebook Likes can accurately predict Big Five personality traits\cite{kosinski2013private}. Results are best summarised in a 2018 meta-analysis which states “digital traces from social media can be studied to assess and predict theoretically distant psycho-social characteristics with remarkable accuracy”\cite{settanni2018predicting}. 

Political ideology has often been neglected as a focus of this kind of inquiry. However, the accurate prediction of ideology from digital footprints could be misused to the detriment of society in several ways.
If it is possible to accurately predict an individual’s ideology from their digital behaviour (even digital behaviour that is not of an explicitly political nature) then individuals with democratic sympathies living in authoritarian regimes may inadvertently reveal their non-conforming political views through ostensibly harmless online behaviour and be at risk of government retaliation. Additionally, the possibility of accurately estimating ideology may enable and encourage online political micro-targeting strategies aimed at voter suppression, which are considered to be in opposition with a functional liberal democracy by some\cite{anderson2018one}. 

This paper seeks to elucidate the extent to which an individual’s political ideology can be determined through records of their online behaviour. We have scraped the usernames and political ideologies of 91,000 users active on Reddit, one of the largest social news and discussion platforms globally. We have also recorded the frequency with which (most of) these users comment and post in a range of interest based discussion sub-forums (`subreddits') as well as the textual content of around 100 comments per user. With this data, we modelled the political ideology of these users as a function of the extent to which they engage with different subreddits and the textual content of their comments. 

Our data was scraped from the \href{https://www.reddit.com/r/PoliticalCompassMemes/}{r/PoliticalCompassMemes} subreddit in which users `humorously' critique ideologies in opposition to their own. In this subreddit, users ‘flair’ their posts with with their results from the popular \href{https://www.politicalcompass.org/test}{Political Compass Test}\footnote{In reality, though users presumably take the test and assign themselves to one of the ideological categories featured in the test, ideological labels should be considered as self-identified ideological placement by users as explained in Section \ref{Data}.}. \fref{fig.pcm-comment-fig} shows an example of how users' comments are flaired with their political ideology. \fref{fig.pcm-post-fig} shows a post from the subreddit in which a user flaired as conservative makes fun of U.S. President Joe Biden. \fref{fig.policompass-fig} shows the political compass; users are assigned to one of the four quadrants in the two dimensional ideological space. These flairs provide an ideological label to which we can map digital footprints. Section \ref{Data} of this paper provides further information on our data. Section \ref{Methodology} details the modelling strategies we employ. 

\begin{figure}[!htbp]
\centering
  \fbox{\includegraphics[width=10cm,height=4.7cm]{Figures/pcm-comment-fig.png}}%
  \caption{A comment from a user who has flaired themselves as having economically right wing views and a response from a user who has flaired themselves as having a `libertarian left' ideology \label{fig.pcm-comment-fig}}
\end{figure}

\begin{figure}[!htbp]
\centering
  \fbox{\includegraphics[width=10cm,height=9.7cm]{Figures/pcm-post-fig.png}}%
  \caption{A post from a user who has flaired themselves as a member of the `authoritarian right' \label{fig.pcm-post-fig}}
\end{figure}


\begin{figure}[!htbp]
\centering
  \fbox{\includegraphics[width=10cm,height=9.7cm]{Figures/policompass-fig.png}}%
  \caption{The political compass. Flaired users take a test specifying the extent to which they agree with politically charged statements (e.g. "If economic globalisation is inevitable, it should primarily serve humanity rather than the interests of trans-national corporations") and are assigned to one of four quadrants: libertarian left (social democrat), libertarian right (libertarian), authoritarian left (communist) or authoritarian right (traditional conservative) depending on their answers \label{fig.policompass-fig}}
\end{figure}

Through developing predictive models we have contributed to the literature on how, through online behaviour, people may implicitly disclose private information through several avenues.

Firstly, existing findings show that binary conceptions of ideology can be accurately predicted from digital footprints. We investigate whether these results hold for our new, original data set but more importantly, we utilise our sophisticated measure of ideology, which allows for centrist self-identification (on both the economic and `social'\footnote{The term `social' for this ideological dimension is somewhat misleading, we provide a fuller explanation of what is meant here in Section \ref{Data}.} dimensions of ideology) to test if the accurate prediction of ideology from digital foot prints is robust to the inclusion of self-identified centrists. In a similar vein, we also illustrate how the quality of predictions is affected by the complexity of the ideological variable we seek to model. Further, our sophisticated response variable allows us to decompose users' ideology into both an economic component and `social' component. This allows us to investigate whether the economic component of political ideology is more readily predictable than the `social' component. To our knowledge, no other study in this field has attempted to answer these questions. Finally, we model ideology using as features the frequency of users' interactions with subreddits, the textual content of their texts and the union of these sets of features. This provides insight into what sorts of digital footprints are most informative with respect to ideology. These results have important policy upshots that we discuss in Section \ref{Discussion}. 

This paper also illustrates the usefulness of Reddit as a source of ‘social data’. The vast majority of studies in this space rely on Twitter and Facebook data. Facebook data is no longer readily available in response to increased public scrutiny over online privacy. Twitter, though a useful source of digital data, only contains textual information. By showing Reddit to be a reliable source of rich social data we hope to spur further developments in this field.

We find that economic ideology is readily predictable from digital footprints and that this result is robust to the inclusion of self-identified economic centrists, although model performance diminishes significantly when centrists are included. Contrastingly, our models are unable to predict `social’ ideology at levels significantly above performance baselines. We also show that classification of a complex dependent variable representing nine different ideological classes can be achieved with a level of accuracy above baseline levels. In all cases, the frequency of interactions with different subreddits (analogous to digital footprints like search logs, purchase histories, etc.) is a stronger predictor than the textual content of comments and the union of both sets of features only marginally improves performance. We provide a fuller account of our results in Section \ref{Results}. 


\chapter{Key Literature}
\label{KeyLiterature}


This chapter will lay out some of the key results in the broader area of ‘social data science’ focused on predicting private traits from digital data. It will also lay out the psychological basis of ideology and attempts at modeling ideology as a function of psychological traits.

\section{Social data science}
\label{KeyLiterature-social-data-science}

There is a growing body of work illustrating how online behaviour implicitly discloses private traits. Pioneers in linking traits to digital behaviour relied on volunteers granting access to their social media information and were thus constrained to relatively small sample sizes \cite{Ross2009, Amichai-Hamburger2010, Golbeck2011a, Gosling2011}. More recently, researchers have begun using larger data sets with thousands of users or posts as the basis of analysis to make more robust findings. It has been shown that sexual orientation can be accurately predicted from pictures of an individual’s face with neural networks\cite{wang2018deep} and that Facebook Likes can accurately predict Big Five personality traits, gender, race, drug use and other traits\cite{kosinski2013private}. Even high level features of a Facebook profile (number of friends, number of statuses posted) have been shown to correlate with and predict personality\cite{10.1145/2380718.2380722}. 

Indeed, it has been found that digital footprints can be used to train statistical models capable of predicting people’s personality traits to a higher degree of accuracy than their close friends and family\cite{youyou2015computer}. Publicly available information from Twitter profiles\cite{Golbeck2011, Quercia2011} and Facebook messages\cite{Schwartz2013} has also been used to predict these traits using natural language processing techniques. Meta analyses claim that “the predictive power of digital footprints over personality traits is in line with the standard “correlational upper-limit” for behavior to predict personality”\cite{Azucar2018} and that psychosocial traits more broadly can be accurately predicted by digital footprints\cite{settanni2018predicting}. 

Further, it is not only digital traces from social media that can be effectively employed to predict private traits. The word choices of blog writers\cite{Yarkoni2010},  the images `favorited' by Flickr users\cite{Segalin2017} and mobile phone usage data\cite{stachl2020predicting} have also be used to predict personality traits. 

These sorts of models can be effectively used to persuade people; S.C. Matz et al., have shown, using Facebook advertising with different messages aimed at people with different ‘Likes’ indicating particular personality types, that engagement with advertised content can be effectively increased through tailoring messages to predicted psychological traits\cite{Matz2017}.

Some attention has been payed to political traits too. Natural language processing techniques can be used to accurately classify the political leanings of Twitter users\cite{colleoni2014echo, Conover2011} and their political engagement or ideological extremity\cite{Preotiuc-Pietro2017}. Hashtags and network analysis of mention/retweet networks can also be leveraged to effectively classify the ideologies of Twitter users\cite{Conover2011}. Kosinski et. al's seminal work\cite{kosinski2013private} pays some attention to political traits. Kosinski et al. map the Likes of 9,572 American Facebook users with a self-disclosed party affiliation of  either Democrat or Republican using a logistic regression model, illustrating that the model’s predictions on unseen data achieve an ROC-AUC (receiver operating characteristic, area under curve) of 0.85. Our approach to modelling ideology as a function of digital footprints broadly based on the methods used in this paper. 

\section{Psychological basis of ideology}
\label{KeyLiterature-psychological}

An individual’s latent psychological makeup drives both their online behaviour and their political beliefs. We believe this provides for the observed association between online behaviour that is not of an explicitly political nature and ideological views (commenting on the \href{https://www.reddit.com/r/Marxism/}{r/Marxism} or \href{https://www.reddit.com/r/Conservative/}{r/Conservative} subreddits would constitute explicitly political online behaviour). There is a documented association between psychological traits and certain interests\cite{Wolfradt2001, McCrae1997}. Interests likely impact language use (if you're into movies you probably use words like `actor' and `film' a lot) and people with certain interests are more likely to participate in subreddits pertaining to these interests. 

Psychological traits also drive ideology. There is a substantive amount of literature in psychology that has focused on modeling ideology as a function of scores on particular psychometric scales. In one study, the Big Five model of personality was used to predict party preferences in Italy, Spain, Germany, Greece and Poland\cite{Vecchione2011}. It was found that they were more powerful predictors than demographic traits (age, gender, income, education) and that openness to experience predicts left wing views whilst conscientiousness predicts voting for conservative parties. They note that the linkage between personality and political views is consistent with theoretical expectations: conscientiousness comprises a preference for order and adherence with rules whereas openness to new ideas correlates against preferences for rigid social hierarchy\cite{Vecchione2011}. It has been shown that including scores from the HEXACO model of personality as additional regressors alongside Big Five traits, increases the proportion of variance explained when modeling ideology\cite{Chirumbolo2010}.

Another study illustrates that scores on Hartmann’s Boundaries Questionnaire can predict conservatism\cite{Hiel2004}. Some results are consistent with theoretical expectations; conservatism is correlated with a preference for rigid and well defined social structures whilst other results are harder to explain; conservatism is also positively correlated with a preference for blurred edges and soft lines in art\cite{Hiel2004}. This suggests the psychological underpinnings of ideological belief may go further than expected. 

More broadly, a meta-analysis of ‘conservatism as a function of social cognition’ has found that death anxiety, system instability, dogmatism, openness to experience, uncertainty tolerance, need for order, structure and closure, integrative complexity, fear of threat and loss and self-esteem all have predictive power of conservatism\cite{Jost2003}. Consider how an individual’s interests and activities are likely influenced by these traits. Someone with substantial death anxiety may resultingly have a strong interest in existential philosophy. Someone with low openness to experience may prefer older, familiar television shows to more recent ones.

Consequently, psychological traits influence both ideology and our interests, which in turn influences our online behaviour, providing for an observable mapping of online behaviour to ideology which can be approximated by statistical learning models. 



==> copyright.tex <==
% https://www.monash.edu/graduate-research/examination/publication
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis/writing-the-thesis-chapters/structuring-a-long-text
\copyrightnotice{

% \addtocontents{toc}{\vspace{1em}}  % Add a gap in the Contents, for aesthetics

\textsuperscript{\textcopyright  \authornames (2021).}

I certify that I have made all reasonable efforts to secure copyright permissions for third-party content included in this thesis and have not knowingly added copyright content to my work without the owner's permission.


}
